A Generalized Cheeger Inequality

The generalized conductance $\phi(G,H)$ between two graphs $G$ and $H$ on the same vertex set $V$ is defined as the ratio $$ \phi(G,H) = \min_{S\subseteq V} \frac{cap_G(S,\bar{S})}{ cap_H(S,\bar{S})}, $$ where $cap_G(S,\bar{S})$ is the total weight of the edges crossing from $S$ to $\bar{S}=V-S$. We show that the minimum generalized eigenvalue $\lambda(L_G,L_H)$ of the pair of Laplacians $L_G$ and $L_H$ satisfies $$ \lambda(L_G,L_H) \geq \phi(G,H) \phi(G)/8, $$ where $\phi(G)$ is the usual conductance of $G$. A generalized cut that meets this bound can be obtained from the generalized eigenvector corresponding to $\lambda(L_G,L_H)$. The inequality complements a recent proof that $\phi(G)$ cannot be replaced by $\Theta(\phi(G,H))$ in the above inequality, unless the Unique Games Conjecture is false.

==> background.tex <==
\section{Preliminaries} \label{sec:background}

In this Section we briefly recall background facts about Laplacians of weighted graphs. For more details, we refer the reader to \cite{RoyleGodsil} and \cite{Boman03support}. Throughout the paper, we discuss connected graphs with positive edge weights. We use $n$ and $m$ to denote $|V|$ and $|E|$.

\subsection{Condition Number and Support}

A symmetric matrix $A$ is positive semi-definite if for any vector $x$, $x^T Ax \geq 0$. For such semi-definite matrices $A$, we can also define the $A$-norm of a vector $x$ by
$$||x||_A^2=x^T A x.$$

Fix an arbitrary numbering of the vertices and edges of a graph $G$. Let $w_{i,j}$ denote the weight of the edge $(i,j)$. The Laplacian $L_G$ of $G$ is the matrix defined by: (i) $L_G(i,j) = -w_{i,j}$, (ii) $L_G(i,i) = \sum_{i\neq j} w_{i,j}$. For any vector $x$, one can check that

$$x^TL_Gx = \sum_{u, v \in E} (x_u-x_v)^2w_{uv}.$$

This definition allows us to define the condition number of a pair of graphs, $\kappa(G, H)$ on the same vertex set as follows:

\[
\kappa(G, H) = \left( \max_{x^T1 =0} \frac{x^TL_Gx}{x^TL_Hx} \right) \cdot \left( \max_{x^T1 =0} \frac{x^TL_Hx}{x^TL_Gx} \right)
\]

The condition number is an algebraically motivated notion; upper bounds on it are used to predict the convergence rate of iterative numerical algorithms.
To ease the analysis of it, we define a one-sided quantity of it known as the support:

\[
\sigma(A/B) = \max_{x^T1 =0} \frac{x^TAx}{x^TBx}
\]

It can be checked that $\kappa(G, H) = \sigma(G/H) \sigma(H/G)$.



%Stolen from SODA04 submission
\subsection{Support Tree Conjugate Gradient}
\label{sec:stcg}

A support tree preconditioner is defined over a potentially larger graph than the one for
which it is created, hence in this section we present the tools
necessary to compare matrices of different sizes.

Let $A$ and
$B = \begin{pmatrix}
T & U\\ U\TT & W
\end{pmatrix}$
be SDD matrices such that $T$ is nonsingular and
both $A$ and $W$ are $n \times n$ matrices.  A case of particular
interest is when both $A$ and $B$ are Laplacians, and $B$ corresponds
to that of a tree with $T$ representing the connectivity among the
internal nodes, $U$ representing the connectivity between the internal
nodes and the leaves, and $W$ a diagonal matrix representing the
degrees of the leaves, which are identified with the vertices of $A$.
In this case we say $B$ is a support tree for $A$.  Gremban's
thesis describes an extension of the preconditioned conjugate
gradient (PCG) method, called support tree conjugate gradient (STCG),
which is designed to handle the case in which we seek to precondition
$A$ with the potentially larger matrix $B$ \cite{Gremban-thesis}.  Gremban
demonstrates the following.

\begin{lemma}\label{lem:stcg}
Given $A$ and $B$ as defined above, if $Q = W - U\TT T\IV U$ then
STCG on $A$ using $B$ as a preconditioner
takes at most $\sqrt{\kappa(A,Q)}\log(1/\epsilon)$ iterations.
\end{lemma}

We call $Q$ the Schur complement of $B$ (with respect to $W$); $Q$ represents
the connectivity among the vertices of $W$ in $B$ at a cost of
greater density than $B$.  STCG is in fact
designed to efficiently simulate invoking PCG with $Q$ as a
preconditioner. The latter requires solving a system of the form
$Q\vv{x} = \vv{b}$ for $\vv{x}$ during each iteration; however, $Q$
may be much more dense than $B$.  STCG finds a solution $\vv{x}$ by
solving $B \begin{pmatrix} \vv{y} \\ \vv{x}\end{pmatrix} =
\begin{pmatrix} \vv{0} \\ \vv{b}\end{pmatrix}$ and simply discarding
$\vv{y}$.

\begin{proposition}If $B \begin{pmatrix} \vv{y} \\ \vv{x}\end{pmatrix} =
\begin{pmatrix} \vv{0} \\ \vv{b}\end{pmatrix}$ then $Q\vv{x} = \vv{b}$.
\end{proposition}

\iffalse
\begin{proof} We have that $T\vv{y} + U\vv{x} = \vv{0}$. Thus $y = -T\IV U\vv{x}$,
and $Q\vv{x} = U\TT\vv{y} + W\vv{x} = b$.\end{proof}\\
\fi

When $B$ is a support tree the system can be solved quite efficiently.
By Lemma~\ref{lem:stcg} we may bound the convergence rate of STCG on
$A$ and $B$ by bounding $\sigma(A / Q)\cdot \sigma(Q / A)$; however,
in our analysis we will find it more convenient to refer directly to
the structure of larger Laplacian $B$, so we introduce the following
definitions.

\iffalse
Let $A$ and $B = \begin{pmatrix}
T & U\\ U\TT & W \end{pmatrix}$ be Laplacians such that
$A$ and $W$ are $n \times n$ matrices,
\fi
Let $A$ and $B$ be defined as above, and let
$\bar{A} = \begin{pmatrix}0 & 0\\0 & A\end{pmatrix}$ be the same size
as $B$.  The matrix $\bar{A}$ allows us to compare $A$ and $B$ and leads
to a natural definition of $\sigma(A / B)$.

\begin{definition}\label{def:supp:AB}
The support of $B$ for
$A$, $\sigma(A / B)$ is $\sigma(\bar{A} / B)$.
\end{definition}

The proposition below, which follows from Proposition 6.1 in Boman and
Hendrickson~\cite{BomanHen2002}, demonstrates that the above definition
is consistent.

\begin{proposition}Given the definitions above, if $T$ is nonsingular then
$\sigma(A / B) = \sigma(A / Q)$.
\end{proposition}

We must take a slightly different approach in defining $\sigma(B / A)$
due to a disparity in the null spaces of $\bar{A}$ and $B$.

\begin{definition}\label{def:supp:BA}
The support of $A$ for $B$, $\sigma(B / A)$ is

$
\min \{\tau \mid \forall \vv{x},\,
\tau\cdot \vv{x}\TT A \vv{x} \geq
\begin{pmatrix} \vv{y} \\ \vv{x} \end{pmatrix}\TT B
\begin{pmatrix} \vv{y} \\ \vv{x} \end{pmatrix}, \text{ where }
\vv{y} = -T\IV U \vv{x}\}.
$
\end{definition}

Although the definition above may not seem as natural as
Definition~\ref{def:supp:AB}, it does capture the notion
of supporting $Q$ with $A$.

\begin{proposition}\label{prop:supp:BA}
We have
$\sigma(B / A) = \sigma(Q / A)$.
\iffalse
\leq
\min \{\tau \mid \forall \vv{x} \forall \vv{y},\,
\tau\cdot \vv{x}\TT A \vv{x} \geq
\begin{pmatrix} \vv{y} \\ \vv{x} \end{pmatrix}\TT B
\begin{pmatrix} \vv{y} \\ \vv{x} \end{pmatrix}\} = \sigma(B / \bar{A}).
\fi
\end{proposition}

\iffalse
\begin{proof} The result follows from the definitions of $\sigma(Q / A)$ and
$\sigma(B / A)$ and the fact that
$$\begin{pmatrix} -T\IV U\vv{x} \\ \vv{x} \end{pmatrix}\TT B
\begin{pmatrix} -T\IV U\vv{x} \\ \vv{x} \end{pmatrix} = \vv{x}\TT Q \vv{x}.$$\end{proof}
\fi

% Local variables:
% TeX-master: "Paper"
% End:


%It follows that $L_G$ is positive semi-definite and $L_G$-norm is a valid norm.

%We also define a partial order $\preceq$ on symmetric semi-definite matrices, where $A \preceq B$ if $B-A$ is positive semi-definite. This definition  is equivalent to $x^TAx \leq x^TBx$ for all $x$. We say that a %graph $H$ {\em $\kappa$-approximates} a graph $G$ if
%$$L_H \preceq L_G  \preceq  \kappa L_H.$$

%By the definition of $\preceq$ from above, this relationship is equivalent to $x^TL_Hx \leq  x^TL_Gx  \leq \kappa x^TL_Hx$ for all vectors $x$. This implies that the {\em condition number} of the pair $(L_G,L_H)$ is upper bounded by $\kappa$. The { condition number} is an algebraically motivated notion; upper bounds on it are used to predict the convergence rate of iterative numerical algorithms.


\subsection{Conductances}

Given a weighted graph $G$ and a subset of its vertices $S \subseteq V$,
we use $Vol_G(S)$ to denote the total weight of all edges with at least
one end point in $S$, and $\delta_G(S, \bar{S})$ to denote the total
weight of all edges with exactly one endpoint in $S$ and one endpoint
in $\bar{S}$.

The conductance of a graph $G$, $\alpha(G)$ can then be defined as:
\[
\alpha(G) = \min_{S \subseteq V, Vol_G(S) \leq \frac{1}{2}Vol_G(V)}
\frac{\delta_G(S, \bar{S})}{Vol_G(S)}
\]

And the relative conductance of graphs $G$ and $H$ on the same vertex set is:
\[
\alpha(G, H) = \min_{S \subseteq V}
\frac{\delta_G(S, \bar{S})}{\delta_H(S, \bar{S})}
\]

It can be checked that the conductance of $G$ is within a constant factor
of the relative conductance of $G$ with the complete demand graph where
$w_H(u, v) = \frac{Vol_G(u) Vol_G(v)}{Vol_G(V)}$.


